BERT Rankers are Brittle: a Study using Adversarial Document Perturbations

Contextual ranking models based on BERT are now well established for a wide range of passage and document ranking tasks. However, the robustness of BERT-based ranking models under adversarial inputs is under-explored. In this paper, we argue that BERT-rankers are not immune to adversarial attacks targeting retrieved documents given a query. Firstly, we propose algorithms for adversarial perturbation of both highly relevant and non-relevant documents using gradient-based optimization methods. The aim of our algorithms is to add/replace a small number of tokens to a highly relevant or non-relevant document to cause a large rank demotion or promotion. Our experiments show that a small number of tokens can already result in a large change in the rank of a document. Moreover, we find that BERT-rankers heavily rely on the document start/head for relevance prediction, making the initial part of the document more susceptible to adversarial attacks. More interestingly, we find a small set of recurring adversarial words that when added to documents result in successful rank demotion/promotion of any relevant/non-relevant document respectively. Finally, our adversarial tokens also show particular topic preferences within and across datasets, exposing potential biases from BERT pre-training or downstream datasets.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> evaluation.tex <==
\section{Evaluation}
In this section we report the overall effectiveness of gradient-based attacking methods against the BERT ranking models. Note that all results are averages on $5$ times random initialization. Our results suggest with only a minor perturbation, the documents encounter significant rank changes. We also conduct a statistical analysis of the selected adversarial tokens by both instance-wise and universal attack algorithm.   

\subsection{Adversarial Attack Effectiveness}
 We firstly add a fixed small number of tokens to the documents beginning. As Figure~\ref{fig:general} shows, for both datasets, such a minor perturbation can demote the top-ranked documents and promote the last-ranked documents by a large margin, compared to the performance of randomly selected tokens. TREC-DL contains short passages and thus it's more sensitive to the input modification than ClueWeb09. On average, a $3$-token difference can promote the passages from rank 100 into top-3 and demote the top-1 ranked passages to the last-five positions. Meanwhile, a $5$-token perturbation on ClueWeb09 documents results in relatively smaller rank changes of around 70. Besides, the instance-wise attacking shows superior performance regarding the rank changes than the universal attacking method. This is not surprising, since the universal adversarial tokens are updated on the documents from all queries, trading off efficiency for better generalization. 

\subsection{Adversarial Attack Ablations}
%\mpara{The number of adversarial tokens vs the attacking effectiveness} 
A rational question to ask is how many tokens needed to cause a prominent prediction difference and meanwhile, meet the constrain of imperceptible perturbation. Thus we experiment with adding a various number of tokens to the start of documents. Figure~\ref{fig:length} presents the rank changes for ClueWeb09 (we omit TREC-DL due to the page limit). It indicates that increasing the number continuously enlarges the rank difference. For lengthy ClueWeb09 documents (contain usually more then 512 tokens), one-token difference is negligible and yet it can already drop the rank for on average 46, indicating the fragility of BERT ranking models. 

%\mpara{The positions of adversarial tokens vs the attacking effectiveness} 
Considering the ranking model might be biased to the top part of the texts, we also conduct an ablation experiment with different perturbing positions 
including the \textbf{start} and the \textbf{end} of the documents (within the $512$ token), the positions where the original tokens have the  \textbf{highest} and the \textbf{lowest} $i$ ($i$=5) gradient scores, the \textbf{random} selected positions and the \textbf{middle} position computed from the text length divided by $2$. Figure~\ref{fig:position} indicates significant position biases of the ranking model. Namely, modifying the start of the texts causes much higher rank changes than the rest positions. This could be related to the input concatenation procedure of query-document pairs. Even though the self-attention module desiderates to mitigate the position bias, the query-document relevance is still highly impacted by the text head which is adjacent to the query, urging a more robust design to avoid such bias. 

\begin{figure}[t!]
      \centering
      \includegraphics[width=0.9\linewidth]{images/global_instance.png}
      \caption{The average rank changes of instance-wise and universal attacking on BERT ranker. We add $5$ and $3$ tokens to the start of ClueWeb09 and TRECT-DL documents respectively. The random bar serves as bottom line. }
      \label{fig:general}
    \end{figure}


\begin{figure*}[t!]
\centering
\begin{subfigure}[b]{0.45\textwidth}
      \centering
      \includegraphics[width=\textwidth]{images/length.png}
      \caption{The average rank changes vs adversarial token lengths.}
      \label{fig:length}
    \end{subfigure}
\begin{subfigure}[b]{0.45\textwidth}
      \centering
      \includegraphics[width=\textwidth]{images/position.png}
      \caption{The average rank changes vs adversarial token positions. }
      \label{fig:position}
    \end{subfigure}
\caption{Ablation study of instance-wise attack on randomly selected $40$ queries from ClueWeb09. we use $5$ tokens for figure (b). }
\end{figure*}   

\subsection{Adversarial Token Analysis}
The instance-wise method generates $i$ adversarial tokens for each query independently. Hypothetically, these tokens should differ from each other if queries are diverse. In this section we conduct an naive statistic analysis of the token frequency to exploit the potential patterns of adversarial token choices.   

\mpara{Rank Demotion} We randomly sample $40$ queries from ClueWeb09 and list the $5$ tokens selected to demote the top-ranked documents in Figure~\ref{fig:heatmap} (due to space limit we omit the rest queries). We can observe frequent occurrences of some particular tokens, such as ``acceptable", even without the universal knowledge. In other words, the ranking model dislikes ``acceptable" no matter what queries it deals with. Besides, we also find ``acceptable" in the 5-token universal trigger. This suggests that repeating the instance-wise attacking algorithm for many times delivers a similar set of adversarial tokens as the universal trigger token. Our experimental results also show that adding $5$ of the most frequent tokens to all top-ranked documents causes on average $83$ rank drop, compared to $79$ by universal triggers.   
%\todo[]{How is the attacking performance of individual trigger tokens compared to the universal triggers?}


\begin{figure}[t!]
      \centering
      \includegraphics[width=1.0\linewidth]{images/Heatmap_inplace_clueweb09_40queries.eps}
      \caption{The five adversarial tokens added to the beginning of the highest-ranked document for 40 queries from ClueWeb09, selected by local ranking attack method to demote the document. Specific tokens frequently recur across queries. The frequency is denoted by the color.}
      \label{fig:heatmap_inplace}
    \end{figure}
    

Explaining the frequent repetition of adversarial tokens is crucial to better understand neural network rankers. Our first intuition of the dataset bias is overturned by the rare appearance of ``acceptable" in our corpus. Another assumption might be due to the pretrained  embeddings and the intriguing correlation between the high-dimensional model parameters. We will leave a more comprehensive explanation attempt to the future work.



\mpara{Rank Promotion} A simple way to enhance the query-document relevance is increasing their textual overlaps. Similarly as above, we also inspected the instance-wise adversarial tokens for rank promotion. Unsurprisingly, we found out that within $5$ tokens, around half of which are query tokens. Apart from that, there are also frequent repetitions of particular tokens across the whole dataset. We visualize all tokens weighted by their frequency for all $200$ queries in Figure~\ref{fig:wordcloud}. As it suggests, natural disaster relevant tokens such as ``tornadoes", ``hurricane" are the most favored by the model for many different queries. Note that the trigger, namely the $5$ tokens selected by the universal attacking are ``hindusim", ``earthquakes", ``childbirth", ``tornadoes" and ``wikipedia", showing a high similarity to the frequent instance-wise adversarial tokens. 
%Although there are a few number of queries related to natural disasters in the dataset, the reason why natural disaster tokens are highly favored by the model still remains opaque. 



\begin{figure}[t!]
      \centering
      \includegraphics[width=0.9\linewidth]{images/Heatmap_frequent_count_topdoc.png}
      \caption{Adversarial tokens from instance-wise attacking for ClueWeb09 document demotion. Specific tokens frequently occurred across queries.}
      \label{fig:heatmap}
    \end{figure}
    
\begin{figure}[t!]
      \centering
      \includegraphics[width=0.8\linewidth]{images/wordcloud.png}
      \caption{Adversarial tokens from instance-wise attacking for ClueWeb09 document promotion. Tokens related to natural disaster are frequently occurred across queries. }
      \label{fig:wordcloud}
    \end{figure}
  


\mpara{Pretraining Bias vs Dataset Bias} Apart from the above-mentioned natural disaster tokens, we also noticed the existence of other topics from the instance-wise adversarial tokens in rank promotion (We omit rank demotion since the tokens don't show prominent topic patterns). We present the appeared tokens (with the threshold of 2 frequency) in a 2D visualization for both datasets and as Figure~\ref{fig:pca} indicates, some tokens related to \textit{nature}, \textit{religion}, \textit{ethnic} and \textit{medicine} are picked simultaneously by both datasets. Since we use the same bert-base-uncased model and fine-tune it on two different down stream datasets, we hypothesize that the model might memorize some bias from the pretraining data. On the other hand, it could be also possible the datasets remain some topic preferences. Figure~\ref{fig:pca} shows that TREC-DL has a strong preference of \textit{ medicine} while for ClueWeb09, \textit{religion} and \textit{nature} are slightly more dominant. Via manual observation of the $200$ queries from ClueWeb09, we found out only $4$ queries relevant to \textit{natures} but $24$ queries about \textit{disease}. For TREC-DL, we leave a more automatic method for topic extraction to future work due to the large training corpus.       

\begin{figure}[t!]
      \centering
      \includegraphics[width=0.9\linewidth]{images/pca_bias.png}
      \caption{Frequently appeared adversarial tokens from instance-wise attacking for both datasets. Note that the topic of each token is manually assigned. }
      \label{fig:pca}
    \end{figure}

==> experiments.tex <==
\section{Adversarial Attacks to Neural Rankers}

\mpara{Model and Datasets} We fine-tune the bert-base-uncased model on (i) ClueWeb09 and (ii) MSMARCO passage ranking datasets by stacking a feed-forward layer on the pooled representation and optimizing the margin loss between positive-negative document pairs. ClueWeb09 contains in total 200 real-world queries and the corresponding $100$ retrieved documents. We conduct the attack experiments on all of the 200 queries. For MSMARCO passage ranking dataset, we include randomly selected 1000 queries from the development set and the 200 queries from the TREC-DL test set (all denoted as TREC-DL for simplicity). Depending on the preference of a particular document, we consider two attack scenarios: (1)\textbf{rank demotion} for a top-ranked document, and (2)\textbf{ rank promotion} for a bottom-ranked document. We employ (i) the \textbf{instance-wise attack} method where we find adversary texts of documents for each query independently, and (ii) the \textbf{universal attack} where the adversarial texts or triggers generalize to all queries. In the following, we introduce the detailed attack methods using rank demotion as the objective.

\mpara{Instance-wise Attack} Given a query \query{} and a text input \doc{} from dataset $\mathcal{D} = \{Q, D\}$ where $q\in Q$ and $d\in D$, the ranking model \model{} computes the relevance score of \doc{} w.r.t \query{} by \model{}$(q, d)$ and the ranking position $\Pi_{d}$ is obtained by comparing all relevance scores of a list of pre-retrieved documents. We intend to craft an adversary example \xdoc{} for \doc{}, by adding $i$ tokens $\mathbf{x} = \{x_1, x_2, \cdots, x_i\}$ or replacing $i$ tokens with $\mathbf{x}$ in $d$, so that the rank difference $|\Pi_{d}-\Pi_{\hat{d}}|$ is maximized. We denote such perturbation by $\hat{d} = d + \mathbf{x}$. Specifically, to demote $d$, we minimize the relevance score (and maximize the score to promote $d$) as following:
\begin{align}
\label{eq:attack-instance}
  \underset{\mathbf{x}}{ \text{arg\, min}} \ \Phi (q, d+\mathbf{x})
   %\text{s.t. } \ \mathtt{dist} (d, \hat{d} ) \leq \epsilon \nonumber
\end{align}
 To ensure imperceptible perturbation, we choose the $i$ to be no more than $20$ in our experiments. Due to the discrete nature of tokens, we adapt HotFlip~\cite{ebrahimi2017hotflip} to approximate the relevance changes induced by tokens from the whole vocabulary $\mathcal{V}$ using the first-order Taylor expansion as equation~\ref{eq:attack-tokens}. Note that $v - x_i$ is element-wise subtraction on the embedding dimension. To search for multiple adversary tokens, we also apply beam search to extract the top $i$ candidate tokens similarly as~\cite{wallace2019universal}. The best $\mathbf{x}$ is realized by repeating equation~\ref{eq:attack-tokens} until the relevance score decreases no more.  

\begin{align}
    \label{eq:attack-tokens}
  \underset{v\in \mathcal{V}}{ \text{arg\, min}} \ [v - x_i]^\top \nabla_{x_i} \Phi (q, d+ x_i)
   %\text{s.t. } \ \mathtt{dist} (d, \hat{d} ) \leq \epsilon \nonumber
\end{align}

\mpara{Universal Attack} Rather than generating adversarial tokens for a particular query-document instance, we aim at finding $\mathbf{x}$ which can generalize to the whole dataset $\mathcal{D}$. Such $\mathbf{x}$ is also called universal trigger. In other words, adding such tokens is able to promote or demote a document for any query in the Dataset. Thus we minimize the relevance score expectation for all queries using equation~\ref{eq:attack-universe}. The searching strategy remains the same as equation~\ref{eq:attack-tokens}. 

\begin{align}
    \label{eq:attack-universe}
  \underset{\mathbf{x}}{ \text{arg\, min}} \ \mathbb{E}_{(q, d) \sim \mathcal{D}} [ \Phi (q, d+ \mathbf{x})]
   %\text{s.t. } \ \mathtt{dist} (d, \hat{d} ) \leq \epsilon \nonumber
\end{align}

\mpara{Metric} We measure the absolute rank change normalized by the ranking size as $\mathtt{NRC} = \frac{|\Pi_d - \Pi_{\hat{d}}|}{|\Pi|}$. Since we only consider the top-100 retrieved documents for both datasets, $|\Pi|$ equals to 100. 


==> figure-token-analysis.tex <==

\begin{figure*}[ht!]
\centering
% \begin{subfigure}[b]{0.35\textwidth}
%       \includegraphics[width=0.9\linewidth]{images/Heatmap_frequent_count_topdoc.png}
%       \caption{heatmap}
%       \label{fig:general}
%  \end{subfigure}     
\begin{subfigure}[b]{0.3\textwidth}
      \centering
      \includegraphics[width=\textwidth]{images/wordcloud.png}
      \caption{word cloud}
      \label{fig:length}
    \end{subfigure}
\begin{subfigure}[b]{0.3\textwidth}
      \centering
      \includegraphics[width=\textwidth]{images/pca_bias.png}
      \caption{ Impact of adversarial token positions }
      \label{fig:pca}
    \end{subfigure}
\caption{Ablation study of instance-wise attack on randomly selected $40$ queries from ClueWeb09. we use $5$ tokens for figure (b). }
\end{figure*}   


==> introduction.tex <==
\section{Introduction}


Deep neural networks (DNNs) are vulnerable under adversarial attacks. Namely, an imperceptible perturbation of the input can mislead a DNN model and cause erroneous prediction. In image applications, adding some noise to the pixels of an image so that it remains identical to humans might completely change the prediction label. In natural language processing (NLP), a natural adversarial input is ensured by either modifying a small number of words, or rephrasing the text using synonyms. Due to the discrete nature of human languages, such small changes might cause a big difference in embedding vectors. Entangling with high-dimension parameters, DNN models are not just sensible to malicious input, but also hard to interpret. Recent work in adversarial attack and defense aims at building stronger machine learning frameworks, as well as exposing the model or dataset biases, which is crucial for developing robust and more importantly, explainable machine learning algorithms.

Recommendation systems on the other hand, have successfully adapted many recent designs from NLP applications. For instance, using the BERT models to measure the query-document relevance has the first time surpassed the traditional BM25 model in information retrieval. However, unlike the well awareness of the fragility of neural models in NLP, the adversarial attacking on neural rankers hasn't been well studied. One reason could be the queries are usually short sequences of terms, modifying the query terms are usually noticeable and unnatural. On the other hand, for ranking tasks, the goal is not predicting an independent label or score, but rather an aggregation of multiple outputs, namely a rank. More specifically, given a query, the ranking model generates a relevance score for each candidate document and the eventual output is a rank of the scores from all documents of interest. Therefore, the attacking objects are different based on the rank position of the specific document. For a middle-ranked document, both increasing and decreasing its rank position are possible, which is not the case for the top-ranked or the last-ranked document. In this paper, we target on perturbing the text documents and only consider rank demotion for the top document and rank promotion for the last document, in order to facilitate the attacking evaluation. 
%Nevertheless in real world, ranking attack has more practical scenarios such as search engine optimization (SEO) which promotes the rank position of web pages. 

Adversarial attack algorithms can be categorized into model agnostic and model introspective. For texts data, the model introspective methods make use of gradient signals to generate adversarial examples. At the expense of losing fluency to some extent, these methods are usually more efficient compared to the model-agnostic algorithms. The generated adversarial artifacts can be input-dependent or universal. That is, instead of generating an instance-wise artifact for each input instance, \citet{wallace2019universal} use the gradient-based attacking method to craft a short text snippet which is optimized on the whole dataset. Such text snippet is called ``universal trigger" and can cause a specific prediction when added to any input instance from the dataset. Despite the lack of natural attribute, the universal triggers raised more concerns in terms of security since it's easy and fast to deploy.

  
In this paper, we intend to bridge the gap between text ranking and adversarial attacking. We apply the well-known gradient-based attacking algorithm HotFlip~\cite{ebrahimi2017hotflip} to generate instance-wise adversarial words (also called tokens) for each input document. Meanwhile, we also borrow the idea from~\cite{wallace2019universal} to obtain the universal triggers which apply to the whole dataset. We conduct attacking experiments against the BERT ranking model on ClueWeb09 and TREC-DL datasets. Our results show that both instance-wise attack and universal triggers can cause significant rank changes, exposing the fragility of BERT rankers. Finally, we also conduct a detailed analysis of the instance-wise adversarial tokens   
and the universal triggers. We find out (1) some instance-wise tokens occur frequently across many different queries, sharing big overlaps with the universal triggers; (2) some adversarial tokens overlap across different datasets, suggesting a pretraining bias; (3) the majority of adversarial tokens fall into a group of sensitive topics like \textit{ethnics}, \textit{diseases} or \textit{natural disasters}, indicating potential dataset biases.  

%In this paper, we study adversarial attacks against Bert-based text ranking models. We borrow the universal trigger from~\citet{wallace2019universal} 




==> related_work.tex <==
\section{Related Work}
\mpara{Adversarial Attacks in NLP} There are two major lines of attacking approaches in NLP tasks such as text classification and natural language inference. The first is without knowing model architectures and parameters, namely under the black-box setup, the attacker uses predefined heuristic rules to generate \textit{natural} (in human perspective) substitutes of words or sentences, so that to fool the victim model. The prevalent heuristics include synonym replacement~\cite{jin2019bert, ren2019generating}, mask-and-fill by contextualized language models~\cite{ li2020contextualized, li2020bert}, human-in-the-loop strategy~\cite{wallace2019trick}, etc. On the other hand, white-box attack assumes full access to model parameters. Thus the attacker can use gradient signals to guide the searching process within a few rounds of forward and backward computation~\cite{ebrahimi2017hotflip, XU2020103641}. Due to the discrete nature of human languages, gradient-based approaches are efficient yet lack of fluency compared to rule-based methods. For more related adversarial attacking methods, we point the reader to recent surveys\cite{zhang2020adversarial, huq2020adversarial}.

\mpara{Universal Triggers} Unlike above methods, \citet{wallace2019universal} generate input-agnostic universal triggers using HotFlip~\cite{ebrahimi2017hotflip} for NLP models and datasets. Triggers are tokens or phrases, injecting such trigger to any input text can mislead the victim model to a target prediction. For high-dimensional neural networks, it's unsurprising to find tokens from a large vocabulary that always result in a particular prediction. Moreover, \citet{wallace2021poisoning} also argue it's possible to plant any trigger in the model by poisoning the training data with a small set of crafted instances containing such trigger. After retraining, the model will pick up the patterns or shortcuts induced by the trigger and make the same prediction whenever the trigger occurs in the input. We are more interested in this universal trigger because it exposes higher potential risks if a single phrase can not only impact the model prediction, but also apply to the whole dataset.

\mpara{Adversarial Attacks in Text Ranking} Fewer efforts have been invested in ranking especially text ranking models. The closest to our work is from~\citet{raval2020one}, where they perturb a top-ranked document given a query by replacing no more than 5 words and observe a significant drop of rank position. They solve the text perturbation in model-agnostic fashion using differential evolution algorithm~\cite{storn1997differential}. Our work is different from theirs in: (i) we use gradient-based method to search candidate tokens to replace and be replaced; (ii) we consider more scenarios such as document demotion and promotion for transformer models and (iii) more importantly, we focus on looking for universal triggers and endeavor to explain the triggers, as an attempt to discover potential dataset and model biases.  
